DeepUQ: Assessing the Aleatoric Uncertainties from two Deep Learning Methods

Assessing the quality of aleatoric uncertainty estimates from uncertainty quantification (UQ) deep learning methods is important in scientific contexts, where uncertainty is physically meaningful and important to characterize and interpret exactly. We systematically compare aleatoric uncertainty measured by two UQ techniques, Deep Ensembles (DE) and Deep Evidential Regression (DER). Our method focuses on both zero-dimensional (0D) and two-dimensional (2D) data, to explore how the UQ methods function for different data dimensionalities. We investigate uncertainty injected on the input and output variables and include a method to propagate uncertainty in the case of input uncertainty so that we can compare the predicted aleatoric uncertainty to the known values. We experiment with three levels of noise. The aleatoric uncertainty predicted across all models and experiments scales with the injected noise level. However, the predicted uncertainty is miscalibrated to $\rm{std}(\sigma_{\rm al})$ with the true uncertainty for half of the DE experiments and almost all of the DER experiments. The predicted uncertainty is the least accurate for both UQ methods for the 2D input uncertainty experiment and the high-noise level. While these results do not apply to more complex data, they highlight that further research on post-facto calibration for these methods would be beneficial, particularly for high-noise and high-dimensional settings.

==> checklist.tex <==
% \Task{open}{open}
% \Task{done}{done}
% \Task{started}{started}


\begin{CheckList}{Goal}
\Goal{open}{Figures: Prior Predictive Check (PPC): Baseline Data}
\begin{CheckList}{Task}
\Task{open}{visualization of example objects based on prior distribution data -- e.g., with different kinds of noise and foreground/etc properties; e.g., multi-panel: grid of objects at different properties; consider 1d and 2d examples}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Figures: Posterior-Prior Comparison}
\begin{CheckList}{Task}
\Task{open}{parity (1-1, truth vs predicted) }
\Task{open}{parity residuals (1-1, truth vs predicted) }
\end{CheckList}
\end{CheckList}



\begin{CheckList}{Goal}
\Goal{open}{Figures: Simulation-based Calibration (SBC)}
\begin{CheckList}{Task}
\Task{open}{SBC: posteriors (for a single variable) or corner plots for multiple co-varying variables}
\Task{open}{SBC: rank histogram}
\Task{open}{SBC: Posterior coverage}
\Task{open}{SBC: CDF Parity (true vs predicted cdf)}
\Task{open}{SBC: Rank Covarianae Histogram (new)}
\Task{open}{SBC: $\ell$-C2ST (new)}
\Task{open}{SBC: TARP (new)}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Figures: Posterior Predictive Check (PPC)}
\begin{CheckList}{Task}
\Task{open}{reconstructed object given examples of new fit parameters}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Figures: Latent Space Overlap (pick one)}
\begin{CheckList}{Task}
\Task{open}{isomap}
\Task{open}{t-sne}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Figures: Local Sensitivity Measures in pixel space (pick one)}
\begin{CheckList}{Task}
\Task{open}{Grad-CAM}
\Task{open}{Saliency map}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Figures: Training History }
\begin{CheckList}{Task}
\Task{open}{Loss/Accuracy history for source and target domains}
\end{CheckList}
\end{CheckList}


\begin{CheckList}{Goal}
\Goal{open}{Metrics}
\begin{CheckList}{Task}
\Task{open}{Final Loss}
\Task{open}{ROC/AUC}
\Task{open}{Correlation coefficient}
\end{CheckList}
\end{CheckList}

\begin{CheckList}{Goal}
\Goal{open}{Tables}
\begin{CheckList}{Task}
\Task{open}{if there's an embedding network, a table of those network properties.}
\Task{open}{list of parameter distributions for training and testing scenarios}
\Task{open}{list of parameter set sizes for each model}
\Task{open}{Average 68\% scatter in the difference between the best-fit parameters for $N$ objects.}
\Task{open}{Performance metrics to compare no-DA and DA training.}
\end{CheckList}
\end{CheckList}
